A high-order energy-conserving semi-Lagrangian discontinuous Galerkin method for the Vlasov-Ampere system

In this paper, we propose a high-order energy-conserving semi-Lagrangian discontinuous Galerkin(ECSLDG) method for the Vlasov-Ampere system. The method employs a semi-Lagrangian discontinuous Galerkin scheme for spatial discretization of the Vlasov equation, achieving high-order accuracy while removing the Courant-Friedrichs-Lewy (CFL) constraint. To ensure energy conservation and eliminate the need to resolve the plasma period, we adopt an energy-conserving time discretization introduced by Liu et al. [J. Comput. Phys., 492 (2023), 112412]. Temporal accuracy is further enhanced through a high-order operator splitting strategy, yielding a method that is high-order accurate in both space and time. The resulting ECSLDG scheme is unconditionally stable and conserves both mass and energy at the fully discrete level, regardless of spatial or temporal resolution. Numerical experiments demonstrate the accuracy, stability, and conservation properties of the proposed method. In particular, the method achieves more accurate enforcement of Gauss's law and improved numerical fidelity over low-order schemes, especially when using a large CFL number.

==> SLDG.tex <==
\section{Project: semi-Lagrangian DG schemes for multiscale advection-diffusion equations}

based on mingchang paper and collaborate with Shimeng.

==> main_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
%\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}
%
%% Title. If the supplement option is on, then "Supplementary Material"
%% is automatically inserted before the title.
%\title{An Example Article\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}
%
%% Authors: full names plus addresses.
%\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL
%  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID
%  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
%\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:


==> schematic_eldg1d_st2.tex <==
\begin{figure}[h!]
\centering
\subfigure[]{
\begin{tikzpicture}[x=1cm,y=1cm]%[scale=1.0]
  \begin{scope}[thick]


   \draw (-3,3) node[fill=white] {};
    \draw (-3,-1) node[fill=white] {};
    \draw[black]                   (-3,0) node[left] {} -- (3,0)
                                        node[right]{$t^{n}$};
    \draw[black] (-3,2) node[left] {$$} -- (3,2)
                                        node[right]{$t^{n+1}$};
     \draw[snake=ticks,segment length=2.4cm] (-2.4,2) -- (0,2) node[above left] {$x_{j-\frac12}$};
     \draw[snake=ticks,segment length=2.4cm] (0,2) -- (2.4,2) node[above right] {$x_{j+\frac12}$};

          \draw[snake=ticks,segment length=2.4cm] (-2.4,0) -- (0,0);
     \draw[snake=ticks,segment length=2.4cm] (0,0) -- (2.4,0);
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \draw[-latex,dashed,red] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
                                        node[black,below]{$x_{j-\frac12}^\star$ };

                \draw[-latex,dashed,red] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
                                        node[black,below right]{ $x_{j+\frac12}^\star$};
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


  %\node[blue, rotate=0] (a) at ( 0.7  ,1.3)  { \tiny $ \frac{d\tilde{x}(t ) }{dt}= a(\tilde{x}(t ),t)$, };
  %\node[blue, rotate=0] (a) at ( 0.7  ,1.3-0.5)  {\tiny   $\tilde{x}(t^{n+1} )={x_{j+\frac12}}$ };

  \node[  rotate=0] (a) at ( 0.6  ,1.3)  { \scriptsize Characteristics tracing };

  \draw[-latex  ](  1.7, 1.1 )node[right=-3pt,scale=1.0]{ }
        to[out=320,in=150] ( 2.1  , 0.8) node[below=2pt] { };

  %{\tiny $\left.\frac{d\tilde{x}(t;x,t^{n+1}) }{dt}= a(\tilde{x}(t;x,t^{n+1}),t)\right|_{x_{j-\frac12}}$ };
  %\node[blue, rotate=0] (a) at (3,1.) {\tiny $\frac{d\tilde{x}(t;x_{j+\frac12},t^{n+1})}{dt}= a(\tilde{x}(t;x_{j+\frac12},t^{n+1}),t)$ };
  \end{scope}
\end{tikzpicture}
 }
 \subfigure[]{
\begin{tikzpicture}[x=1cm,y=1cm]%[scale=1.0]
  \begin{scope}[thick]


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            \draw[-latex,dashed,red] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
%                                        node[black,below]{  };
%
%                \draw[-latex,dashed,red] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
%                                        node[black,below right]{ };
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    \draw[white,fill=blue!4] (0,2) -- (-0.8,0)  -- (2,0) -- (2.4, 2)
      -- cycle;
    \node[blue!80, rotate=0] (a) at ( 1. ,1.5 ) {\Large $\Omega_{j}$ };




   \draw (-3,3) node[fill=white] {};
    \draw (-3,-1) node[fill=white] {};
    \draw[black]                   (-3,0) node[left] {} -- (3,0)
                                        node[right]{$t^{n}$};
    \draw[black] (-3,2) node[left] {$$} -- (3,2)
                                        node[right]{$t^{n+1}$};
     \draw[snake=ticks,segment length=2.4cm] (-2.4,2) -- (0,2) node[above left] {$x_{j-\frac12}$};
     \draw[snake=ticks,segment length=2.4cm] (0,2) -- (2.4,2) node[above right] {$x_{j+\frac12}$};

          \draw[snake=ticks,segment length=2.4cm] (-2.4,0) -- (0,0);
     \draw[snake=ticks,segment length=2.4cm] (0,0) -- (2.4,0);
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            \draw[-latex,dashed,blue] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
%                                        node[black,below]{$x_{j-\frac12}^\star$ };
%
%                \draw[-latex,dashed,blue] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
%                                        node[black,below right]{ $x_{j+\frac12}^\star$};


  \draw[-latex, blue] (0.,2) node[left] {$$} -- (-1.5+0.7,0)  node[black,below]{$x_{j-\frac12}^\star$ };

  \draw[-latex, blue] (2.4,2) node[left] {$$} -- (1.6+0.4,0)  node[black,below right]{ $x_{j+\frac12}^\star$};



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \draw[-latex,blue!50,dashed] (0.6,2) node[left] {$$} -- (-0.8+0.25*2.8 ,0)
                                        node[black,below]{ };
  \draw[-latex,blue!50,dashed] (1.2,2) node[left] {$$} -- (-0.8+0.5*2.8 ,0)
                                        node[black,below]{ };
  \draw[-latex,blue!50,dashed] (1.8,2) node[left] {$$} -- (-0.8+0.75*2.8 ,0)
                                        node[black,below]{ };

%%%%%%%%%%%%%%%%
\draw[-latex,thick,blue](0.4,1)node[right,scale=1.]{\footnotesize $\tilde{I}_j(t)$}
        to[out=180,in=0] (-0.4,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����

\draw[-latex,thick,blue](1.3,1)node[right,scale=1.]{ }
        to[out=0,in=180] (2.2,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����





  \node[blue, rotate=67] (a) at (-0.7 ,1.) { $\nu_{j-\frac12}$ };
  \node[blue, rotate=80] (a) at (2.5,1.) { $\nu_{j+\frac12}$ };


  \end{scope}
\end{tikzpicture}
 }
\caption{Illustration for the  space-time region of the alternative ELDG formulation. %\QQ{Merge two figures into one}
 }
\label{st2}
\end{figure}


==> schematic_eldg2d.tex <==


\begin{figure}
\centering
%\includegraphics[width=120mm]{illustration_eldg2d}
\begin{tikzpicture}[scale=0.7]
       \begin{scope}[
            yshift= 0,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]
 \draw[black,fill=black!10] (1,4)  -- ( 1,2)  -- (3.5,2) -- (2.8 ,4)       -- cycle;
  \node[black!100, rotate=0] (a) at ( 2.5,2.5) {  $ \tilde{A}_j^{(0)} $ };
    \coordinate (A) at (1,2);
     \coordinate (B) at (3.5,2);
      \coordinate (C) at (2.8,4);
       \coordinate (D) at (1,4);
    %\draw[-latex,thick]  (3,3) node[right,scale=1.0]{}--(A)  node[] {};
    \end{scope}
  % the bottom layer, the mesh at t^n
    \begin{scope}[
            yshift=0,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]
          \draw[step=1.5cm, black] (0,0) grid (4.5,4.5); %defining grids

        %\draw[black,very thick] (0,0) rectangle (5,5);%marking borders
        \coordinate (V) at (3.5,  2);

    \end{scope}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{scope}[
            yshift= 50,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]


        %\draw[black,very thick] (0,0) rectangle (5,5);%marking borders
  \draw[blue,fill=blue!10] (0.5*1+0.5*1.5,  0.5*2+0.5*1.5) -- ( 0.5*3.5+0.5*3, 0.5*2+0.5*1.5)  -- ( 2.8*0.5+0.5*3,4*0.5+3*0.5) -- (1.5*0.5+1*0.5 ,3*0.5+4*0.5)       -- cycle;
  \node[blue!100, rotate=0] (a) at ( 2.6,2.2) {  $\tilde{A}_j(t)$ };


    \coordinate (U) at (0.5*3.5+0.5*3, 0.5*2+0.5*1.5);

    \end{scope}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{scope}[
            yshift= 100,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]
          \draw[step=1.5cm, black ] (1.5,1.5) grid (3,3); %defining grids

        %\draw[black,very thick] (0,0) rectangle (5,5);%marking borders
  \draw[black,fill=black!5] (1.5,1.5)  -- ( 3,1.5)  -- (3,3) -- (1.5 ,3)       -- cycle;
  \node[black!80, rotate=0] (a) at ( 2.6,2.2) {  $ A_j $ };

    \draw[-latex,blue]  (1.5,1.5) node[right,scale=1.0]{}--(A)  node[] {};
    \draw[-latex, blue]  (3,1.5) node[right,scale=1.0]{}--(B)  node[] {};
    \draw[-latex,dashed,blue]  (3,3) node[right,scale=1.0]{}--(C)  node[] {};
    \draw[-latex, blue]  (1.5,3) node[right,scale=1.0]{}--(D)  node[] {};

\coordinate (W) at (3,  1.5);

    \end{scope}
    \begin{scope}[
            yshift= 0,xshift= -80,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]
     \coordinate (O) at (0,0,0);
  \draw[thick,->] (0,0,0) -- (1,0,0) node[anchor=north east]{ };
  \draw[thick,->] (0,0,0) -- (0,1,0) node[anchor=north west]{ };
  \draw[thick,->] (0,0,0) -- (0,0,-3) node[anchor=north]{ };
  \end{scope}

      \begin{scope}[
            yshift= 0,xshift= -80
            ]
            \node[ rotate=0] (a) at ( -1,0.2) {  $y$ };
            \node[ rotate=0] (a) at ( 1 ,0.2) {  $x$ };
            \node[rotate=0] (a) at ( 0.2 ,1) {  $t$ };

  \end{scope}

  \begin{scope}
  [
            yshift= 0,xshift= 120
            ]
            %\draw[step=2cm, black,thick ] (2,2) grid (4,4); %defining grids

    \draw[black,thick ] (3,3)node[below left,scale=1.0]{  $(x_j^l,y_j^b )$}
     -- ( 6,3) node[below right,scale=1.0]{   $(x_j^r,y_j^b)$}
      -- (6,6)node[above right,scale=1.0]{   $(x_{j}^r,y_{j}^t)$}
       -- ( 3 ,6)  node[above left,scale=1.0]{  $(x_{j}^l,y_{j}^t )$}     -- cycle;


\draw[-latex] (5,1) -- (5,1+1) node[left]{ $\eta$ };
  \draw[-latex] (5,1) -- (5+1,1) node[below]{ $\xi$ };

\draw[-latex, blue]  (U)  node[] {} to[out=10,in=180] (2,4.2) node[right,scale=1.0]{} ;
   \draw[-latex, black]  (W)  node[] {} to[out=10,in=180] (2,4.7) node[right,scale=1.0]{} ;
\draw[-latex, black]  (V)  node[] {} to[out=10,in=180] (2,3.7) node[right,scale=1.0]{} ;
  \end{scope}

\end{tikzpicture}
\caption{Illustration for the mapping between dynamic element $\tilde{A}_j(t)$ (left) and the iso-parametric element (right).   }
\label{2dmap}
\end{figure}


==> schematic_sldg1d.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[x=0.9cm,y=1cm]%[scale=1.0]
  \begin{scope}[thick]

  \draw[white,fill=blue!4] (0.,2) to[out=240,in=85] (-1.5+0.7,0) -- (1.6+0.4,0) to[out=85,in=245] (2.4,2)
      -- cycle;
   %\node[blue!70, rotate=0] (a) at ( 1. ,1.5) {\LARGE $\Omega_j$ };
   \draw (-3,3) node[fill=white] {};
    \draw (-3,-1) node[fill=white] {};
    \draw[black]                   (-3,0) node[left] {} -- (3,0)
                                        node[right]{$t^{n}$};
    \draw[black] (-3,2) node[left] {$$} -- (3,2)
                                        node[right]{$t^{n+1}$};
     \draw[snake=ticks,segment length=2.4cm] (-2.4,2) -- (0,2) node[above left] {$x_{j-\frac12}$};
     \draw[snake=ticks,segment length=2.4cm] (0,2) -- (2.4,2) node[above right] {$x_{j+\frac12}$};

          \draw[snake=ticks,segment length=2.4cm] (-2.4,0) -- (0,0);
     \draw[snake=ticks,segment length=2.4cm] (0,0) -- (2.4,0);
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
            \draw[-latex,dashed,blue] (0.,2) node[left] {$$} to[out=240,in=85] (-1.5+0.7,0)
                                        node[black,below]{$x_{j-\frac12}^\star$ };

                \draw[-latex,dashed,blue] (2.4,2) node[left] {$$} to[out=245,in=85] (1.6+0.4,0)
                                        node[black,below right]{ $x_{j+\frac12}^\star$};
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw [decorate,color=red,decoration={brace,mirror,amplitude=9pt},xshift=0pt,yshift=0pt]
(-1.5+0.7,0) -- (1.6+0.4,0) node [red,midway,xshift=0cm,yshift=-20pt]
{\footnotesize $\widetilde{I}_j(t^{n}) = I_{j}^\star$};

\draw [decorate,color=red,decoration={brace,amplitude=10pt},xshift=0pt,yshift=0pt]
(0,2) -- (2.4,2) node [red,midway,xshift=0cm,yshift=20pt]
{\footnotesize $\widetilde{I}_j(t^{n+1}) = I_{j}$};
\draw[-latex,thick,blue](0.2,1)node[right,scale=1.]{$\widetilde{I}_j(t)$}
        to[out=180,in=0] (-0.55 ,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����

\draw[-latex,thick,blue](1.1,1)node[right,scale=1.]{ }
        to[out=0,in=180] (2.1,1) node[above left=2pt] {$$};  %%%thick ʵ�ߣ� dashed ����

  \node[blue, rotate=0] (a) at (-2.  ,1.3)  { \tiny $ \frac{d\tilde{x}(t ) }{dt}= a(\tilde{x}(t ),t)$ };
  \node[blue, rotate=0] (a) at (-2  ,1.3-0.5)  {\tiny where $\tilde{x}(t^{n+1} )={x_{j-\frac12}}$ };

  \draw[-latex,blue ]( -1, 1.3 )node[right=-3pt,scale=1.0]{ }
        to[out=340,in=160] ( -0.5, 1.1) node[below=2pt] { };

  %{\tiny $\left.\frac{d\tilde{x}(t;x,t^{n+1}) }{dt}= a(\tilde{x}(t;x,t^{n+1}),t)\right|_{x_{j-\frac12}}$ };
  %\node[blue, rotate=0] (a) at (3,1.) {\tiny $\frac{d\tilde{x}(t;x_{j+\frac12},t^{n+1})}{dt}= a(\tilde{x}(t;x_{j+\frac12},t^{n+1}),t)$ };
  \end{scope}
\end{tikzpicture}
\label{schematic_1d}
\caption{Illustration for the space-time region for the SLDG formulation.  }
\end{figure}

